Graph Neural Networks for Virtual Sensing in Complex Systems: Addressing Heterogeneous Temporal Dynamics

Real-time condition monitoring is crucial for the reliable and efficient operation of complex systems. However, relying solely on physical sensors can be limited due to their cost, placement constraints, or inability to directly measure certain critical parameters. Virtual sensing addresses these limitations by leveraging readily available sensor data and system knowledge to estimate inaccessible parameters or infer system states. The increasing complexity of industrial systems necessitates deployments of sensors with diverse modalities to provide a comprehensive understanding of system states. These sensors capture data at varying frequencies to monitor both rapid and slowly varying system dynamics, as well as local and global state evolutions of the systems. This leads to heterogeneous temporal dynamics, which, particularly under varying operational end environmental conditions, pose a significant challenge for accurate virtual sensing. To address this, we propose a Heterogeneous Temporal Graph Neural Network (HTGNN) framework. HTGNN explicitly models signals from diverse sensors and integrates operating conditions into the model architecture. We evaluate HTGNN using two newly released datasets: a bearing dataset with diverse load conditions for bearing load prediction and a year-long simulated dataset for predicting bridge live loads. Our results demonstrate that HTGNN significantly outperforms established baseline methods in both tasks, particularly under highly varying operating conditions. These results highlight HTGNN's potential as a robust and accurate virtual sensing approach for complex systems, paving the way for improved monitoring, predictive maintenance, and enhanced system performance. Our code and data are available under https://github.com/EPFL-IMOS/htgnn.

==> tabs/bearing/split_by_rot_ci_bracket.tex <==
\begin{table}[bthp]
\centering
\caption{MAPE comparison across rotational speed categories for $F_x$ and $F_y$}
\label{tab:mape_comparison_rotational_speed}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{llcccccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{6}{c}{\textbf{Rotational Speed [rpm]}} & \multirow{2}{*}{\textbf{Avg.}} & \multirow{2}{*}{\textbf{Std.}}\\
\cmidrule(lr){2-7}
 & \textbf{Model} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} & \\
\midrule

\multirow{5}{*}{\textbf{MAPE\textsubscript{\(F_x\)} (\%)}} 
  & \textbf{LSTM}  &  \underline{2.32} & \underline{3.64} & 3.79 & \underline{2.60} & \underline{3.16} & \underline{3.10} & 0.64 \\
  & \textbf{CNN}   & 5.24 &  6.81 &  7.17 &  4.26 &  4.92 &  5.68 &  1.26 \\
  & \textbf{1D-GCNN}  & 5.94 &  4.99 &  5.66 &  4.90 &  5.90 &  5.48 &  \underline{0.50} \\
  & \textbf{MTGAT} &  2.81 &  6.53 & \underline{2.90} &  4.11 & 3.27 &  3.93 & 1.55 \\
  & \textbf{HTGNN} & \textbf{1.16} & \textbf{1.51} & \textbf{1.81} & \textbf{1.37} & \textbf{0.67} & \textbf{1.30} & \textbf{0.43} \\
\midrule
\multirow{5}{*}{\textbf{MAPE\textsubscript{\(F_y\)} (\%)}} 
  & \textbf{LSTM}  &  \underline{3.98} & 2.03 & 1.85 &  2.59 &  5.53 & 3.20 & 1.55 \\
  & \textbf{CNN}   &  4.84 &  3.64 &  2.61 &  2.83 &  4.95 &  3.77 & \underline{1.09} \\
  & \textbf{1D-GCNN}  & 6.74 &  4.97 &  5.02 &  4.76 &  9.07 &  6.11 &  1.83 \\
  & \textbf{MTGAT} & 4.10 & \underline{1.57} & \underline{1.30} & \underline{1.83} & \underline{3.67} & \underline{2.49} & 1.29 \\
  & \textbf{HTGNN} & \textbf{2.53} & \textbf{1.39} & \textbf{0.66} & \textbf{0.91} & \textbf{1.58} & \textbf{1.42} & \textbf{0.73} \\

\bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[bthp]
\centering
\renewcommand{\arraystretch}{1.1} % Increase line spacing
\caption{
Model performance (MAPE) for bearing load predictions ($F_x$ and $F_y$) across different rotational speeds. Values in parentheses indicate the 95\% maximum MAPE observed across five runs.}
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{lllllllr}
\toprule
\multirow{2}{*}{} & & \multicolumn{5}{c}{\textbf{Rotational Speed [r/min]}} & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){3-7}
        & \textbf{Model} & \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40} & \textbf{50} & \\
\midrule
\multirow{5}{*}{\textbf{MAPE\textsubscript{\(F_x\)} (\%)}} 
        & \textbf{LSTM} & \underline{2.4} (6.4) &  \underline{3.8} (17.1) &  3.9 (16.3) &   \underline{2.7} (8.1) &  \underline{3.3} (10.4) &  \underline{3.2} \\
        & \textbf{1D-CNN} &  5.4 (13.3) &  7.1 (28.4) &  7.4 (29.8) &  4.4 (12.2) &  5.2 (16.8) &  5.9 \\
        & \textbf{1D-GCNN} & 3.9 (13.2) &  4.4 (14.8) &  5.8 (17.5) &  3.2 (10.5) &  5.3 (16.7) &  4.5 \\
        & \textbf{MTGAT} &   2.9 (9.3) &  6.9 (35.5) &   \underline{3.0} (9.1) &  4.2 (20.9) &  3.4 (10.6) &  4.1 \\
        & \textbf{HTGNN} &  \textbf{0.9} (2.9) &   \textbf{1.1} (3.3) &   \textbf{1.4} (8.9) &   \textbf{1.0} (2.9) &  \textbf{0.7} (2.1) &  \textbf{1.0} \\
\midrule
\multirow{5}{*}{\textbf{MAPE\textsubscript{\(F_y\)} (\%)}} 
        & \textbf{LSTM} & \underline{4.2} (19.1) &   2.1 (5.8) &   1.9 (5.6) &   2.7 (7.4) &  5.8 (18.8) &  3.3 \\
        & \textbf{1DCNN} &  5.1 (20.8) &  3.8 (15.7) &   2.7 (5.3) &   3.0 (9.3) &  5.2 (12.3) &  4.0 \\
        & \textbf{1D-GCNN} &  6.0 (21.8) &  3.8 (12.5) &  4.4 (12.2) &  4.0 (15.5) &  8.3 (29.7) &  5.3 \\
        & \textbf{MTGAT} &  4.3 (18.6) &   \underline{1.6} (4.9) &   \underline{1.4} (4.4) &   \underline{1.9} (6.4) &  \underline{3.8} (10.7) &  \underline{2.6} \\
        & \textbf{HTGNN} &   \textbf{2.1} (8.6) &   \textbf{1.2} (6.4) &   \textbf{0.7} (1.9) &   \textbf{1.1} (4.4) &   \textbf{1.1} (4.2) &  \textbf{1.2} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tabs/bridge/nrmse_by_temp_std.tex <==
\begin{table}[bthp]
\centering
\caption{NRMSE Comparison Across Temperature Categories} 
\label{tab:nrmse_comparison} 
\renewcommand{\arraystretch}{1.1} % Increase line spacing
\scalebox{0.9}{
    \begin{tabularx}{1.08\linewidth}{l *{6}{c}} 
    \toprule
        & \multicolumn{4}{c}{\textbf{Temperature (°C)}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Avg.}}} \\
    \cmidrule(lr){2-5}
    \textbf{Model} & \textbf{$<$ 0} & \textbf{0-10} & \textbf{10-20} & \textbf{$>$ 20} & \\
    \midrule
    \textbf{LSTM}   & 0.089 \tiny{$\pm$ 0.059} & \underline{0.054} \tiny{$\pm$ 0.037} & 0.046 \tiny{$\pm$ 0.038} & 0.049 \tiny{$\pm$ 0.037} & 0.059 \tiny{$\pm$ 0.043} \\
    \textbf{1D-CNN} & 0.125 \tiny{$\pm$ 0.079} & 0.066 \tiny{$\pm$ 0.057} & \textbf{0.043} \tiny{$\pm$ 0.033} & 0.049 \tiny{$\pm$ 0.038} & 0.070 \tiny{$\pm$ 0.052} \\
    \textbf{1D-GCNN}  & \underline{0.080} \tiny{$\pm$ 0.054} & \underline{0.054} \tiny{$\pm$ 0.038} & 0.045 \tiny{$\pm$ 0.037} & \textbf{0.046} \tiny{$\pm$ 0.036} & 0.056 \tiny{$\pm$ 0.041} \\
    \textbf{MTGAT}  & 0.118 \tiny{$\pm$ 0.094} & 0.095 \tiny{$\pm$ 0.088} & 0.047 \tiny{$\pm$ 0.037} & 0.052 \tiny{$\pm$ 0.045} & 0.078 \tiny{$\pm$ 0.066} \\
    \textbf{HTGNN}  & \textbf{0.072} \tiny{$\pm$ 0.041} & \textbf{0.048} \tiny{$\pm$ 0.031} & \underline{0.044} \tiny{$\pm$ 0.036} & \underline{0.047} \tiny{$\pm$ 0.038} & \textbf{0.053} \tiny{$\pm$ 0.037} \\
    \bottomrule
    \end{tabularx}
}
\end{table}



